Tensor-based Subspace Factorization for StyleGAN

In this paper, we propose $\tau$GAN a tensor-based method for modeling the latent space of generative models. The objective is to identify semantic directions in latent space. To this end, we propose to fit a multilinear tensor model on a structured facial expression database, which is initially embedded into latent space. We validate our approach on StyleGAN trained on FFHQ using BU-3DFE as a structured facial expression database. We show how the parameters of the multilinear tensor model can be approximated by Alternating Least Squares. Further, we introduce a tacked style-separated tensor model, defined as an ensemble of style-specific models to integrate our approach with the extended latent space of StyleGAN. We show that taking the individual styles of the extended latent space into account leads to higher model flexibility and lower reconstruction error. Finally, we do several experiments comparing our approach to former work on both GANs and multilinear models. Concretely, we analyze the expression subspace and find that the expression trajectories meet at an apathetic face that is consistent with earlier work. We also show that by changing the pose of a person, the generated image from our approach is closer to the ground truth than results from two competing approaches.

==> fig/accv_legacy/Fig7/fig7.tex <==
% \documentclass{standalone}
% \usepackage{graphicx}  
% \usepackage{subcaption}
% \begin{document}

% \begin{figure}[h!]
% \centering    
% \begin{subfigure}{.30\linewidth}
% \includegraphics[width=\linewidth]{tex/fig/Fig7/config_alphaals_noreg_hat.png}
%% \caption{vectorised Model}  
% \end{subfigure}
% \begin{subfigure}{.30\linewidth}
% \includegraphics[width=\linewidth]{tex/fig/Fig7/config_alphaals_noreg_true.png}
%% \caption{Reference Image}  
% \end{subfigure}
% \begin{subfigure}{.30\linewidth}
% \includegraphics[width=\linewidth]{tex/fig/Fig7/config_alphaals_noreg_hat_ext.png}
%% \caption{Extended Model}  
% \end{subfigure}
%% \caption{Comparing the vectorised model to the extended model}
% \end{figure} 


% %%%%%%%%%%%%%%%%
% %%% BEFORE Stella changed some minor things (06.07.2020)
% \begin{figure}[htb]
% \centering    
% \begin{subfigure}{.45\linewidth}
%     \begin{subfigure}{.30\linewidth}
%     \includegraphics[width=\linewidth]{tex/fig/Fig7/config_alphaals_noreg_hat.png}
%   %% \caption{vectorised Model}  
%     \end{subfigure}
%     \begin{subfigure}{.30\linewidth}
%     \includegraphics[width=\linewidth]{tex/fig/Fig7/config_alphaals_noreg_true.png}
%   %% \caption{Reference Image}  
%     \end{subfigure}
%     \begin{subfigure}{.30\linewidth}
%     \includegraphics[width=\linewidth]{tex/fig/Fig7/config_alphaals_noreg_hat_ext.png}
%   %% \caption{Extended Model}  
%     \end{subfigure}
%     \caption{BU3D-FE data points (out of training sample)}
% \end{subfigure}
% \begin{subfigure}{.45\linewidth}
%      \begin{subfigure}{.30\linewidth}
%     \includegraphics[width=\linewidth]{tex/fig/Fig7/config_alphaals_noreg_hat_obama.png}
%   % \caption{vectorised Model}  
%     \end{subfigure}
%     \begin{subfigure}{.30\linewidth}
%     \includegraphics[width=\linewidth]{tex/fig/Fig7/config_alphaals_noreg_true_obama.png}
%   % \caption{Reference Image}  
%     \end{subfigure}
%     \begin{subfigure}{.30\linewidth}
%     \includegraphics[width=\linewidth]{tex/fig/Fig7/config_alphaals_noreg_hat_ext_obama.png}
%   % \caption{Extended Model}  
%     \end{subfigure}
    
%     \begin{subfigure}{.30\linewidth}
%     \includegraphics[width=\linewidth]{tex/fig/Fig7/config_alphaals_noreg_hat_mona.png}
%   % \caption{vectorised Model}  
%     \end{subfigure}
%     \begin{subfigure}{.30\linewidth}
%     \includegraphics[width=\linewidth]{tex/fig/Fig7/config_alphaals_noreg_true_mona.png}
%   % \caption{Reference Image}  
%     \end{subfigure}
%     \begin{subfigure}{.30\linewidth}
%     \includegraphics[width=\linewidth]{tex/fig/Fig7/config_alphaals_noreg_hat_ext_mona.png}
%   % \caption{Extended Model}  
%     \end{subfigure}
%     \caption{Arbitrary reference images.}
% \end{subfigure}
% \caption{\red{If you can read this, a suitable caption has not been written yet.}}
% \label{fig:fig7}
% \end{figure} 

%%%%%%%%%%%%%%%%
%%% AFTER Stella changed some minor things (06.07.2020)
\begin{figure}[htb]
\centering
%%%%%%%%% vectorisED 
    \begin{subfigure}{.24\linewidth}
    \includegraphics[width=\linewidth]{fig/accv_legacy/Fig7/config_alphaals_noreg_hat.png}
    \\
    \includegraphics[width=\linewidth]{fig/accv_legacy/Fig7/config_alphaals_noreg_hat_obama.png}\\
     \includegraphics[width=\linewidth]{fig/accv_legacy/Fig7/config_alphaals_noreg_hat_mona.png}
    \caption{Vectorised}
    \label{subfig:vectorised}
    \end{subfigure}
%%%%%%%%%%%%%%%%
    \begin{subfigure}{.24\linewidth}
    \includegraphics[width=\linewidth]{fig/accv_legacy/Fig7/config_alphaals_noreg_hat_ext.png}\\
    \includegraphics[width=\linewidth]{fig/accv_legacy/Fig7/config_alphaals_noreg_hat_ext_obama.png}\\
    \includegraphics[width=\linewidth]{fig/accv_legacy/Fig7/config_alphaals_noreg_hat_ext_mona.png}
    \caption{Style-Separated}     
%    \caption{Extended Model} 
    \label{subfig:extended}
    \end{subfigure}
%%%%%%%%%%%%%%%% REFERENCE    
    \begin{subfigure}{.24\linewidth}
    \includegraphics[width=\linewidth]{fig/accv_legacy/Fig7/config_alphaals_noreg_true.png}
    \\
     \includegraphics[width=\linewidth]{fig/accv_legacy/Fig7/config_alphaals_noreg_true_obama.png}\\
    \includegraphics[width=\linewidth]{fig/accv_legacy/Fig7/config_alphaals_noreg_true_mona.png}     
    \caption{Reference Image}
    \label{subfig:reference}
    \end{subfigure}
\caption{Reconstruction examples of the \subref{subfig:reference} ground truth images, resulting from either \subref{subfig:vectorised} the vectorised model, or \subref{subfig:extended} the style-separated model. The top row shows an in-sample example, while rows two and three illustrate arbitrary reference images. 
%\red{If you can read this, a suitable caption has not been written yet.}
}
\label{fig:fig7}
\end{figure} 

% \end{document}

==> fig/accv_legacy/Fig7/fig7a-insample.tex <==
\begin{figure}[hbt]
\centering    
\begin{subfigure}{.30\linewidth}
    \red{plot another identity}
    \includegraphics[width=\linewidth]{Fig7/config_alphaals_noreg_hat.png}
    \caption{Vectorised Model}  
\end{subfigure}
\begin{subfigure}{.30\linewidth}
    \includegraphics[width=\linewidth]{Fig7/config_alphaals_noreg_true.png}
    \caption{Reference Image}  
\end{subfigure}
\begin{subfigure}{.30\linewidth}
    \includegraphics[width=\linewidth]{Fig7/config_alphaals_noreg_hat_ext.png}
    \caption{Extended Model}  
\end{subfigure}
\caption{Comparing the vectorised model to the extended model}
\label{fig:vec_vs_extended_model}
\end{figure} 

==> fig/accv_legacy/Fig9/fig9.tex <==


\begin{figure}[tb]  
\centering
\begin{subfigure}{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{fig/accv_legacy/Fig9/F0002/true.png}  
\caption{Ground Truth}\label{fig9:true}
\end{subfigure}
\begin{subfigure}{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{fig/accv_legacy/Fig9/F0002/ols.png}  
\caption{Non-regularised}\label{fig9:ols}
\end{subfigure}
\begin{subfigure}{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{fig/accv_legacy/Fig9/F0002/reg.png}  
\caption{Regularised}\label{fig9:reg}
\end{subfigure}

\begin{subfigure}{.49\linewidth}
\centering
%\rotatebox[]{90}{OLS}
\includegraphics[width=\linewidth]{fig/accv_legacy/Fig9/F0002/OLSexp.png}  
\includegraphics[width=\linewidth]{fig/accv_legacy/Fig9/F0002/OLSexp_true.png}  
\includegraphics[width=\linewidth]{fig/accv_legacy/Fig9/F0002/L2exp.png}  
\caption{Expression Transfer}\label{fig9:exp}
\end{subfigure}
\begin{subfigure}{.49\linewidth}
\centering
\includegraphics[width=\linewidth]{fig/accv_legacy/Fig9/F0002/OLSrot.png}  
\includegraphics[width=\linewidth]{fig/accv_legacy/Fig9/F0002/OLSrot_true.png}  
\includegraphics[width=\linewidth]{fig/accv_legacy/Fig9/F0002/L2rot.png}  
\caption{Rotation Transfer}\label{fig9:rot}
\end{subfigure}
% Figure  \ref{fig9:true}, \ref{fig9:ols} and \ref{fig9:reg}.  
\caption{\subref{fig9:true} Ground truth approximated by \subref{fig9:ols} the non-regularised model, and \subref{fig9:reg} the regularised model.
In \subref{fig9:exp} and \subref{fig9:rot} the top images are the non-regularised solutions, middle is ground truth and bottom is the regularised solution. }
\label{fig:fig9}
\end{figure}





























% \documentclass{standalone}
% % \usepackage{tikz}
% \usepackage{graphicx}
% % \usepackage{subcaption}

% \begin{document}
%     \includegraphics{transf_true0}
%     \includegraphics{transf_true1}   
%     \includegraphics[{reconstruction}  
%     \includegraphics{transf0} 
%     \includegraphics{transf1} 
% \end{document}

% \documentclass{standalone}
% \usepackage{subcaption}
% \usepackage{todonotes}
% \usepackage{graphicx}
% \begin{document}

% \begin{figure}[htb]  
%     \centering
%     \begin{subfigure}{.66\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{Fig9/reconstruction}  
%     \caption{Reconstruction (OLS)}
%     \end{subfigure}
    
%     \begin{subfigure}{.33\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{Fig9/transf_true0}  
%     \includegraphics[width=\linewidth]{Fig9/transf_true1}  
%     \caption{Ground Truth}
%     \end{subfigure}
%     \begin{subfigure}{.33\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{Fig9/transf0} 
%     \includegraphics[width=\linewidth]{Fig9/transf1} 
%     \caption{Transfer}
%     \end{subfigure}
%     \caption{text}
%     \end{figure}
% \end{document}

